Flow-Based Visual Stream Compression for Event Cameras

As the use of neuromorphic, event-based vision sensors expands, the need for compression of their output streams has increased. While their operational principle ensures event streams are spatially sparse, the high temporal resolution of the sensors can result in high data rates from the sensor depending on scene dynamics. For systems operating in communication-bandwidth-constrained and power-constrained environments, it is essential to compress these streams before transmitting them to a remote receiver. Therefore, we introduce a flow-based method for the real-time asynchronous compression of event streams as they are generated. This method leverages real-time optical flow estimates to predict future events without needing to transmit them, therefore, drastically reducing the amount of data transmitted. The flow-based compression introduced is evaluated using a variety of methods including spatiotemporal distance between event streams. The introduced method itself is shown to achieve an average compression ratio of 2.81 on a variety of event-camera datasets with the evaluation configuration used. That compression is achieved with a median temporal error of 0.48 ms and an average spatiotemporal event-stream distance of 3.07. When combined with LZMA compression for non-real-time applications, our method can achieve state-of-the-art average compression ratios ranging from 10.45 to 17.24. Additionally, we demonstrate that the proposed prediction algorithm is capable of performing real-time, low-latency event prediction.

==> bibliography/ref.tex <==
%Are High-Resolution Event Cameras Really Needed?
@article{gehrig2022high,
  title={Are high-resolution event cameras really needed?},
  author={Gehrig, Daniel and Scaramuzza, Davide},
  journal={arXiv preprint arXiv:2203.14672},
  year={2022}
}

%Real-Time, High-Speed Video Decompression Using a Frame- and Event-Based DAVIS Sensor	
@inproceedings{brandli2014real,
  title={Real-time, high-speed video decompression using a frame-and event-based DAVIS sensor},
  author={Brandli, Christian and Muller, Lorenz and Delbruck, Tobi},
  booktitle={2014 IEEE International Symposium on Circuits and Systems (ISCAS)},
  pages={686--689},
  year={2014},
  organization={IEEE}
}

%Lossless Compression of Neuromorphic Vision Sensor Data Based on Point Cloud Representation
@article{martini2022lossless,
  title={Lossless compression of neuromorphic vision sensor data based on point cloud representation},
  author={Martini, Maria and Adhuran, Jayasingam and Khan, Nabeel},
  journal={IEEE Access},
  volume={10},
  pages={121352--121364},
  year={2022},
  publisher={IEEE}
}

%Spike coding for dynamic vision sensors
@inproceedings{bi2018spike,
  title={Spike coding for dynamic vision sensors},
  author={Bi, Zhichao and Dong, Siwei and Tian, Yonghong and Huang, Tiejun},
  booktitle={2018 Data Compression Conference},
  pages={117--126},
  year={2018},
  organization={IEEE}
}

%Spike coding for dynamic vision sensor in intelligent driving
@article{dong2018spike,
  title={Spike coding for dynamic vision sensor in intelligent driving},
  author={Dong, Siwei and Bi, Zhichao and Tian, Yonghong and Huang, Tiejun},
  journal={IEEE Internet of Things Journal},
  volume={6},
  number={1},
  pages={60--71},
  year={2018},
  publisher={IEEE}
}

%Lossless compression of data from static and mobile dynamic vision sensors-performance and trade-offs
@article{khan2020lossless,
  title={Lossless compression of data from static and mobile dynamic vision sensors-performance and trade-offs},
  author={Khan, Nabeel and Iqbal, Khurram and Martini, Maria G},
  journal={IEEE Access},
  volume={8},
  pages={103149--103163},
  year={2020},
  publisher={IEEE}
}

%Time-aggregation-based lossless video encoding for neuromorphic vision sensor data
@article{khan2020time,
  title={Time-aggregation-based lossless video encoding for neuromorphic vision sensor data},
  author={Khan, Nabeel and Iqbal, Khurram and Martini, Maria G},
  journal={IEEE Internet of Things Journal},
  volume={8},
  number={1},
  pages={596--609},
  year={2020},
  publisher={IEEE}
}

% Event Data Stream Compression Based on Point Cloud Representation
@inproceedings{huang2023event,
  title={Event Data Stream Compression Based on Point Cloud Representation},
  author={Huang, Bowen and Ebrahimi, Touradj},
  booktitle={2023 IEEE International Conference on Image Processing (ICIP)},
  pages={3120--3124},
  year={2023},
  organization={IEEE}
}

@inproceedings{gehrig2021raft,
  title={E-raft: Dense optical flow from event cameras},
  author={Gehrig, Mathias and Millh{\"a}usler, Mario and Gehrig, Daniel and Scaramuzza, Davide},
  booktitle={2021 International Conference on 3D Vision (3DV)},
  pages={197--206},
  year={2021},
  organization={IEEE}
}

%Lossy event compression based on image-derived quad trees and poisson disk sampling
@inproceedings{banerjee2021lossy,
  title={Lossy event compression based on image-derived quad trees and poisson disk sampling},
  author={Banerjee, Srutarshi and Wang, Zihao W and Chopp, Henry H and Cossairt, Oliver and Katsaggelos, Aggelos K},
  booktitle={2021 IEEE International Conference on Image Processing (ICIP)},
  pages={2154--2158},
  year={2021},
  organization={IEEE}
}

%A Novel Approach for Neuromorphic Vision Data Compression based on Deep Belief Network
@article{khaidem2022novel,
  title={A Novel Approach for Neuromorphic Vision Data Compression based on Deep Belief Network},
  author={Khaidem, Sally and Sharma, Mansi and Nevatia, Abhipraay},
  journal={arXiv preprint arXiv:2210.15362},
  year={2022}
}

%Lossless Compression of Event Camera Frames
@article{schiopu2022lossless,
  title={Lossless compression of event camera frames},
  author={Schiopu, Ionut and Bilcu, Radu Ciprian},
  journal={IEEE Signal Processing Letters},
  volume={29},
  pages={1779--1783},
  year={2022},
  publisher={IEEE}
}

%Entropy Coding-based Lossless Compression of Asynchronous Event Sequences
@inproceedings{schiopu2023entropy,
  title={Entropy Coding-based Lossless Compression of Asynchronous Event Sequences},
  author={Schiopu, Ionut and Bilcu, Radu Ciprian},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={3922--3929},
  year={2023}
}

%Low-Complexity Lossless Coding of Asynchronous Event Sequences for Low-Power Chip Integration
@article{schiopu2022low2,
  title={Low-Complexity Lossless Coding of Asynchronous Event Sequences for Low-Power Chip Integration},
  author={Schiopu, Ionut and Bilcu, Radu Ciprian},
  journal={Sensors},
  volume={22},
  number={24},
  pages={10014},
  year={2022},
  publisher={MDPI}
}

%Low-Complexity Lossless Coding for Memory-Efficient Representation of Event Camera Frames
@article{schiopu2022low,
  title={Low-complexity lossless coding for memory-efficient representation of event camera frames},
  author={Schiopu, Ionut and Bilcu, Radu Ciprian},
  journal={IEEE Sensors Letters},
  volume={6},
  number={11},
  pages={1--4},
  year={2022},
  publisher={IEEE}
}

%Evaluation of the impact of lossy compression on event camera-based computer vision tasks
@inproceedings{huang2023evaluation,
  title={Evaluation of the impact of lossy compression on event camera-based computer vision tasks},
  author={Huang, Bowen and Nachtigall Lazzarotto, Davi and Ebrahimi, Touradj},
  booktitle={Applications of Digital Image Processing XLVI},
  year={2023}
}

%Asynchronous spatiotemporal spike metric for event cameras
@article{li2021asynchronous,
  title={Asynchronous spatiotemporal spike metric for event cameras},
  author={Li, Jianing and Fu, Yihua and Dong, Siwei and Yu, Zhaofei and Huang, Tiejun and Tian, Yonghong},
  journal={IEEE Transactions on Neural Networks and Learning Systems},
  year={2021},
  publisher={IEEE}
}

% ARMS and hARMS/fARMS
@article{akolkar2020real,
  title={Real-time high speed motion prediction using fast aperture-robust event-driven visual flow},
  author={Akolkar, Himanshu and Ieng, Sio-Hoi and Benosman, Ryad},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume={44},
  number={1},
  pages={361--372},
  year={2020},
  publisher={IEEE}
}

@article{stumpp2021harms,
  title={hARMS: A Hardware Acceleration Architecture for Real-Time Event-Based Optical Flow},
  author={Stumpp, Daniel C and Akolkar, Himanshu and George, Alan D and Benosman, Ryad B},
  journal={arXiv preprint arXiv:2112.06772},
  year={2021}
}



% datasets



@article{mueggler2017event,
  title={The event-camera dataset and simulator: Event-based data for pose estimation, visual odometry, and SLAM},
  author={Mueggler, Elias and Rebecq, Henri and Gallego, Guillermo and Delbruck, Tobi and Scaramuzza, Davide},
  journal={The International Journal of Robotics Research},
  volume={36},
  number={2},
  pages={142--149},
  year={2017},
  publisher={SAGE Publications Sage UK: London, England}
}

% E-RAFT/DSEC


%RAFT
@inproceedings{teed2020raft,
  title={Raft: Recurrent all-pairs field transforms for optical flow},
  author={Teed, Zachary and Deng, Jia},
  booktitle={Computer Vision--ECCV 2020: 16th European Conference, Glasgow, UK, August 23--28, 2020, Proceedings, Part II 16},
  pages={402--419},
  year={2020},
  organization={Springer}
}

% EDFlow
@article{liu2022edflow,
  title={EDFLOW: Event driven optical flow camera with keypoint detection and adaptive block matching},
  author={Liu, Min and Delbruck, Tobi},
  journal={IEEE Transactions on Circuits and Systems for Video Technology},
  volume={32},
  number={9},
  pages={5776--5789},
  year={2022},
  publisher={IEEE}
}

@incollection{bresenham1998algorithm,
  title={Algorithm for computer control of a digital plotter},
  author={Bresenham, Jack E},
  booktitle={Seminal graphics: pioneering efforts that shaped the field},
  pages={1--6},
  year={1998}
}

@article{alakuijala2018brotli,
  title={Brotli: A general-purpose data compressor},
  author={Alakuijala, Jyrki and Farruggia, Andrea and Ferragina, Paolo and Kliuchnikov, Eugene and Obryk, Robert and Szabadka, Zoltan and Vandevenne, Lode},
  journal={ACM Transactions on Information Systems (TOIS)},
  volume={37},
  number={1},
  pages={1--30},
  year={2018},
  publisher={ACM New York, NY, USA}
}

@ARTICLE{10.3389/fnins.2016.00035,
AUTHOR={Giulioni, Massimiliano and Lagorce, Xavier and Galluppi, Francesco and Benosman, Ryad B.},
TITLE={Event-Based Computation of Motion Flow on a Neuromorphic Analog Neural Platform},      
JOURNAL={Frontiers in Neuroscience},      
VOLUME={10},     
PAGES={35},     
YEAR={2016},      
URL={https://www.frontiersin.org/article/10.3389/fnins.2016.00035},       
DOI={10.3389/fnins.2016.00035},      
ISSN={1662-453X},   
ABSTRACT={Estimating the speed and direction of moving objects is a crucial component of agents behaving in a dynamic world. Biological organisms perform this task by means of the neural connections originating from their retinal ganglion cells. In artificial systems the optic flow is usually extracted by comparing activity of two or more frames captured with a vision sensor. Designing artificial motion flow detectors which are as fast, robust, and efficient as the ones found in biological systems is however a challenging task. Inspired by the architecture proposed by Barlow and Levick in 1965 to explain the spiking activity of the direction-selective ganglion cells in the rabbit's retina, we introduce an architecture for robust optical flow extraction with an analog neuromorphic multi-chip system. The task is performed by a feed-forward network of analog integrate-and-fire neurons whose inputs are provided by contrast-sensitive photoreceptors. Computation is supported by the precise time of spike emission, and the extraction of the optical flow is based on time lag in the activation of nearby retinal neurons. Mimicking ganglion cells our neuromorphic detectors encode the amplitude and the direction of the apparent visual motion in their output spiking pattern. Hereby we describe the architectural aspects, discuss its latency, scalability, and robustness properties and demonstrate that a network of mismatched delicate analog elements can reliably extract the optical flow from a simple visual scene. This work shows how precise time of spike emission used as a computational basis, biological inspiration, and neuromorphic systems can be used together for solving specific tasks.}
}


@inproceedings{Finateu20200Pipeline,
    title = {{0 A 1280×720 Back-Illuminated Stacked Temporal Contrast Event-Based Vision Sensor with 4.86{$\mu$}m Pixels, 1.066GEPS Readout, Programmable Event-Rate Controller and Compressive Data-Formatting Pipeline}},
    year = {2020},
    booktitle = {Digest of Technical Papers - IEEE International Solid-State Circuits Conference},
    author = {Finateu, Thomas and Niwa, Atsumi and Matolin, Daniel and Tsuchimoto, Koya and Mascheroni, Andrea and Reynaud, Etienne and Mostafalu, Pooria and Brady, Frederick and Chotard, Ludovic and Legoff, Florian and Takahashi, Hirotsugu and Wakabayashi, Hayato and Oike, Yusuke and Posch, Christoph},
    volume = {2020-February},
    doi = {10.1109/ISSCC19947.2020.9063149},
    issn = {01936530}
}

@article{Lichtsteiner2008ASensor,
    title = {{A 128 × 128 120 dB 15 {$\mu$}s latency asynchronous temporal contrast vision sensor}},
    year = {2008},
    journal = {IEEE Journal of Solid-State Circuits},
    author = {Lichtsteiner, Patrick and Posch, Christoph and Delbruck, Tobi},
    number = {2},
    volume = {43},
    doi = {10.1109/JSSC.2007.914337},
    issn = {00189200}
}

@article{Brandli2014ASensor,
    title = {{A 240 × 180 130 dB 3 {$\mu$}s latency global shutter spatiotemporal vision sensor}},
    year = {2014},
    journal = {IEEE Journal of Solid-State Circuits},
    author = {Brandli, Christian and Berner, Raphael and Yang, Minhao and Liu, Shih Chii and Delbruck, Tobi},
    number = {10},
    volume = {49},
    doi = {10.1109/JSSC.2014.2342715},
    issn = {00189200}
}

@inproceedings{Son2017ARepresentation,
    title = {{A 640×480 dynamic vision sensor with a 9µm pixel and 300Meps address-event representation}},
    year = {2017},
    booktitle = {Digest of Technical Papers - IEEE International Solid-State Circuits Conference},
    author = {Son, Bongki and Suh, Yunjae and Kim, Sungho and Jung, Heejae and Kim, Jun Seok and Shin, Changwoo and Park, Keunju and Lee, Kyoobin and Park, Jinman and Woo, Jooyeon and Roh, Yohan and Lee, Hyunku and Wang, Yibing and Ovsiannikov, Ilia and Ryu, Hyunsurk},
    volume = {60},
    doi = {10.1109/ISSCC.2017.7870263},
    issn = {01936530}
}

@inproceedings{Posch2011ACDS,
    title = {{A QVGA 143 dB dynamic range frame-free PWM image sensor with lossless pixel-level video compression and time-domain CDS}},
    year = {2011},
    booktitle = {IEEE Journal of Solid-State Circuits},
    author = {Posch, Christoph and Matolin, Daniel and Wohlgenannt, Rainer},
    number = {1},
    volume = {46},
    doi = {10.1109/JSSC.2010.2085952},
    issn = {00189200}
}

@inproceedings{Delbruck2010Activity-drivenSensors,
    title = {{Activity-driven, event-based vision sensors}},
    year = {2010},
    booktitle = {ISCAS 2010 - 2010 IEEE International Symposium on Circuits and Systems: Nano-Bio Circuit Fabrics and Systems},
    author = {Delbr{\"{u}}ck, Tobi and Linares-Barranco, Bernabe and Culurciello, Eugenio and Posch, Christoph},
    doi = {10.1109/ISCAS.2010.5537149}
}

@article{Benosman2012AsynchronousFlow,
    title = {{Asynchronous frameless event-based optical flow}},
    year = {2012},
    journal = {Neural Networks},
    author = {Benosman, Ryad and Ieng, Sio Hoi and Clercq, Charles and Bartolozzi, Chiara and Srinivasan, Mandyam},
    volume = {27},
    doi = {10.1016/j.neunet.2011.11.001},
    issn = {08936080}
}

@article{Clady2014AsynchronousTime-to-contact,
    title = {{Asynchronous visual event-based time-to-contact}},
    year = {2014},
    author = {Clady, Xavier and Clercq, Charles and Ieng, Sio-Hoi and Houseini, Fouzhan and Randazzo, Marco and Natale, Lorenzo and Bartolozzi, Chiara and Benosman, Ryad and Koziol, Scott M},
    url = {www.frontiersin.org},
    doi = {10.3389/fnins.2014.00009},
    keywords = {computer vision, event-based computation, neuromophic vision, robotics, time to contact}
}

@inproceedings{Milde2015BioinspiredFlow,
    title = {{Bioinspired event-driven collision avoidance algorithm based on optic flow}},
    year = {2015},
    booktitle = {Proceedings of 1st International Conference on Event-Based Control, Communication and Signal Processing, EBCCSP 2015},
    author = {Milde, Moritz B. and Bertrand, Olivier J.N. and Benosmanz, Ryad and Egelhaaf, Martin and Chicca, Elisabetta},
    doi = {10.1109/EBCCSP.2015.7300673}
}


@inproceedings{Liu2019AdaptiveSensors,
    title = {{Adaptive time-slice block-matching optical flow algorithm for dynamic vision sensors}},
    year = {2019},
    booktitle = {British Machine Vision Conference 2018, BMVC 2018},
    author = {Liu, Min and Delbruck, Tobi}
}

@inproceedings{Liu2017Block-matchingImplementation,
    title = {{Block-matching optical flow for dynamic vision sensors: Algorithm and FPGA implementation}},
    year = {2017},
    booktitle = {Proceedings - IEEE International Symposium on Circuits and Systems},
    author = {Liu, Min and Delbruck, Tobi},
    doi = {10.1109/ISCAS.2017.8050295},
    issn = {02714310}
}

@article{Horn1981DeterminingFlow,
    title = {{Determining optical flow}},
    year = {1981},
    journal = {Artificial Intelligence},
    author = {Horn, Berthold K.P. and Schunck, Brian G.},
    number = {1-3},
    month = {8},
    pages = {185--203},
    volume = {17},
    publisher = {Elsevier},
    doi = {10.1016/0004-3702(81)90024-2},
    issn = {00043702}
}

@inproceedings{Zhu2018EV-FlowNet:Cameras,
    title = {{EV-FlowNet: Self-Supervised Optical Flow Estimation for Event-based Cameras}},
    year = {2018},
    booktitle = {Robotics: Science and Systems XIV},
    author = {Zhu, Alex and Yuan, Liangzhe and Chaney, Kenneth and Daniilidis, Kostas},
    month = {6},
    publisher = {Robotics: Science and Systems Foundation},
    isbn = {978-0-9923747-4-7},
    doi = {10.15607/RSS.2018.XIV.062}
}

@article{Rueckauer2016EvaluationSensor,
    title = {{Evaluation of event-based algorithms for optical flow with ground-truth from inertial measurement sensor}},
    year = {2016},
    journal = {Frontiers in Neuroscience},
    author = {Rueckauer, Bodo and Delbruck, Tobi},
    number = {APR},
    volume = {10},
    doi = {10.3389/fnins.2016.00176},
    issn = {1662453X}
}

@inproceedings{Aung2018Event-basedFPGA,
    title = {{Event-based Plane-fitting Optical Flow for Dynamic Vision Sensors in FPGA}},
    year = {2018},
    booktitle = {Proceedings - IEEE International Symposium on Circuits and Systems},
    author = {Aung, Myo Tun and Teo, Rodney and Orchard, Garrick},
    volume = {2018-May},
    doi = {10.1109/ISCAS.2018.8351588},
    issn = {02714310}
}

@article{Gallego2020Event-basedSurvey,
    title = {{Event-based Vision: A Survey}},
    year = {2020},
    journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
    author = {Gallego, Guillermo and Delbruck, Tobi and Orchard, Garrick Michael and Bartolozzi, Chiara and Taba, Brian and Censi, Andrea and Leutenegger, Stefan and Davison, Andrew and Conradt, Jorg and Daniilidis, Kostas and Scaramuzza, Davide},
    doi = {10.1109/tpami.2020.3008413},
    issn = {0162-8828}
}

@article{Benosman2014Event-basedFlow,
    title = {{Event-based visual flow}},
    year = {2014},
    journal = {IEEE Transactions on Neural Networks and Learning Systems},
    author = {Benosman, Ryad and Clercq, Charles and Lagorce, Xavier and Ieng, Sio Hoi and Bartolozzi, Chiara},
    number = {2},
    volume = {25},
    doi = {10.1109/TNNLS.2013.2273537},
    issn = {2162237X}
}

@inproceedings{lucas1981iterative,
  title={An iterative image registration technique with an application to stereo vision},
  author={Lucas, Bruce D and Kanade, Takeo and others},
  year={1981},
  organization={Vancouver, British Columbia}
}

@article{Boahen2000Point-to-pointEvents,
    title = {{Point-to-point connectivity between neuromorphic chips using address events}},
    year = {2000},
    journal = {IEEE Transactions on Circuits and Systems II: Analog and Digital Signal Processing},
    author = {Boahen, Kwabena A.},
    number = {5},
    volume = {47},
    doi = {10.1109/82.842110},
    issn = {10577130}
}

@article{Akolkar2020Real-timeFlow,
    title = {{Real-time high speed motion prediction using fast aperture-robust event-driven visual flow}},
    year = {2020},
    journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
    author = {Akolkar, Himanshu and Ieng, Sio Hoi and Benosman, Ryad},
    doi = {10.1109/TPAMI.2020.3010468},
    issn = {0162-8828}
}

@article{Mueggler2017TheSLAM,
    title = {{The event-camera dataset and simulator: Event-based data for pose estimation, visual odometry, and SLAM}},
    year = {2017},
    journal = {International Journal of Robotics Research},
    author = {Mueggler, Elias and Rebecq, Henri and Gallego, Guillermo and Delbruck, Tobi and Scaramuzza, Davide},
    number = {2},
    volume = {36},
    doi = {10.1177/0278364917691115},
    issn = {17413176}
}

@article{Zhu2018ThePerception,
    title = {{The Multivehicle Stereo Event Camera Dataset: An Event Camera Dataset for 3D Perception}},
    year = {2018},
    journal = {IEEE Robotics and Automation Letters},
    author = {Zhu, Alex Zihao and Thakur, Dinesh and {\"{O}}zaslan, Tolga and Pfrommer, Bernd and Kumar, Vijay and Daniilidis, Kostas},
    number = {3},
    volume = {3},
    doi = {10.1109/LRA.2018.2800793},
    issn = {23773766}
}

@misc{Xilinx2018Zynq-7000Sheet,
    title = {{Zynq-7000 SoC Data Sheet}},
    year = {2018},
    author = {{Xilinx}},
    month = {7},
    volume = {DS190}
}

@manual{XilinxZynqDatasheet,
    organization  = {Xilinx},
    title         = {Zynq-7000 SoC Data Sheet: Overview},
    number        = {DS190},
    year          =  {2018},
    month         =  {7},    
    note          = {Rev. 1.11.1},
    url = {https://www.xilinx.com/support/documentation/data\_sheets/ds190-Zynq-7000-Overview.pdf},
}



% inherent compression performed by event cameras
@inproceedings{brandli2014real,
  title={Real-time, high-speed video decompression using a frame-and event-based DAVIS sensor},
  author={Brandli, Christian and Muller, Lorenz and Delbruck, Tobi},
  booktitle={2014 IEEE International Symposium on Circuits and Systems (ISCAS)},
  pages={686--689},
  year={2014},
  organization={IEEE}
}



@inproceedings{freeman2021lossy,
  title={Lossy Compression for Integrating Event Cameras},
  author={Freeman, Andrew C and Mayer-Patel, Ketan},
  booktitle={2021 Data Compression Conference (DCC)},
  pages={53--62},
  year={2021},
  organization={IEEE}
}


@article{blalock2018sprintz,
  title={Sprintz: Time series compression for the internet of things},
  author={Blalock, Davis and Madden, Samuel and Guttag, John},
  journal={Proceedings of the ACM on Interactive, Mobile, Wearable and Ubiquitous Technologies},
  volume={2},
  number={3},
  pages={1--23},
  year={2018},
  publisher={ACM New York, NY, USA}
}



@inproceedings{Finateu20200Pipeline,
    title = {{0 A 1280×720 Back-Illuminated Stacked Temporal Contrast Event-Based Vision Sensor with 4.86{$\mu$}m Pixels, 1.066GEPS Readout, Programmable Event-Rate Controller and Compressive Data-Formatting Pipeline}},
    year = {2020},
    booktitle = {Digest of Technical Papers - IEEE International Solid-State Circuits Conference},
    author = {Finateu, Thomas and Niwa, Atsumi and Matolin, Daniel and Tsuchimoto, Koya and Mascheroni, Andrea and Reynaud, Etienne and Mostafalu, Pooria and Brady, Frederick and Chotard, Ludovic and Legoff, Florian and Takahashi, Hirotsugu and Wakabayashi, Hayato and Oike, Yusuke and Posch, Christoph},
    volume = {2020-February},
    doi = {10.1109/ISSCC19947.2020.9063149},
    issn = {01936530}
}

@article{Lichtsteiner2008ASensor,
    title = {{A 128 × 128 120 dB 15 {$\mu$}s latency asynchronous temporal contrast vision sensor}},
    year = {2008},
    journal = {IEEE Journal of Solid-State Circuits},
    author = {Lichtsteiner, Patrick and Posch, Christoph and Delbruck, Tobi},
    number = {2},
    volume = {43},
    doi = {10.1109/JSSC.2007.914337},
    issn = {00189200}
}

@inproceedings{Son2017ARepresentation,
    title = {{A 640×480 dynamic vision sensor with a 9µm pixel and 300Meps address-event representation}},
    year = {2017},
    booktitle = {Digest of Technical Papers - IEEE International Solid-State Circuits Conference},
    author = {Son, Bongki and Suh, Yunjae and Kim, Sungho and Jung, Heejae and Kim, Jun Seok and Shin, Changwoo and Park, Keunju and Lee, Kyoobin and Park, Jinman and Woo, Jooyeon and Roh, Yohan and Lee, Hyunku and Wang, Yibing and Ovsiannikov, Ilia and Ryu, Hyunsurk},
    volume = {60},
    doi = {10.1109/ISSCC.2017.7870263},
    issn = {01936530}
}

@inproceedings{Posch2011ACDS,
    title = {{A QVGA 143 dB dynamic range frame-free PWM image sensor with lossless pixel-level video compression and time-domain CDS}},
    year = {2011},
    booktitle = {IEEE Journal of Solid-State Circuits},
    author = {Posch, Christoph and Matolin, Daniel and Wohlgenannt, Rainer},
    number = {1},
    volume = {46},
    doi = {10.1109/JSSC.2010.2085952},
    issn = {00189200}
}

@inproceedings{Delbruck2010Activity-drivenSensors,
    title = {{Activity-driven, event-based vision sensors}},
    year = {2010},
    booktitle = {ISCAS 2010 - 2010 IEEE International Symposium on Circuits and Systems: Nano-Bio Circuit Fabrics and Systems},
    author = {Delbr{\"{u}}ck, Tobi and Linares-Barranco, Bernabe and Culurciello, Eugenio and Posch, Christoph},
    doi = {10.1109/ISCAS.2010.5537149}
}

@article{Benosman2012AsynchronousFlow,
    title = {{Asynchronous frameless event-based optical flow}},
    year = {2012},
    journal = {Neural Networks},
    author = {Benosman, Ryad and Ieng, Sio Hoi and Clercq, Charles and Bartolozzi, Chiara and Srinivasan, Mandyam},
    volume = {27},
    doi = {10.1016/j.neunet.2011.11.001},
    issn = {08936080}
}

@article{Clady2014AsynchronousTime-to-contact,
    title = {{Asynchronous visual event-based time-to-contact}},
    year = {2014},
    author = {Clady, Xavier and Clercq, Charles and Ieng, Sio-Hoi and Houseini, Fouzhan and Randazzo, Marco and Natale, Lorenzo and Bartolozzi, Chiara and Benosman, Ryad and Koziol, Scott M},
    url = {www.frontiersin.org},
    doi = {10.3389/fnins.2014.00009},
    keywords = {computer vision, event-based computation, neuromophic vision, robotics, time to contact}
}

@inproceedings{Milde2015BioinspiredFlow,
    title = {{Bioinspired event-driven collision avoidance algorithm based on optic flow}},
    year = {2015},
    booktitle = {Proceedings of 1st International Conference on Event-Based Control, Communication and Signal Processing, EBCCSP 2015},
    author = {Milde, Moritz B. and Bertrand, Olivier J.N. and Benosmanz, Ryad and Egelhaaf, Martin and Chicca, Elisabetta},
    doi = {10.1109/EBCCSP.2015.7300673}
}


@article{Horn1981DeterminingFlow,
    title = {{Determining optical flow}},
    year = {1981},
    journal = {Artificial Intelligence},
    author = {Horn, Berthold K.P. and Schunck, Brian G.},
    number = {1-3},
    month = {8},
    pages = {185--203},
    volume = {17},
    publisher = {Elsevier},
    doi = {10.1016/0004-3702(81)90024-2},
    issn = {00043702}
}



@inproceedings{Aung2018Event-basedFPGA,
    title = {{Event-based Plane-fitting Optical Flow for Dynamic Vision Sensors in FPGA}},
    year = {2018},
    booktitle = {Proceedings - IEEE International Symposium on Circuits and Systems},
    author = {Aung, Myo Tun and Teo, Rodney and Orchard, Garrick},
    volume = {2018-May},
    doi = {10.1109/ISCAS.2018.8351588},
    issn = {02714310}
}

@inproceedings{lucas1981iterative,
  title="An iterative image registration technique with an application to stereo vision",
  author={Lucas, Bruce D and Kanade, Takeo and others},
  year={1981},
  organization={Vancouver, British Columbia}
}



@misc{Xilinx2018Zynq-7000Sheet,
    title = {{Zynq-7000 SoC Data Sheet}},
    year = {2018},
    author = {{Xilinx}},
    month = {7},
    volume = {DS190}
}

@manual{XilinxZynqDatasheet,
    organization  = {Xilinx},
    title         = {Zynq-7000 SoC Data Sheet: Overview},
    number        = {DS190},
    year          =  {2018},
    month         =  {7},    
    note          = {Rev. 1.11.1},
    url = {https://www.xilinx.com/support/documentation/data\_sheets/ds190-Zynq-7000-Overview.pdf},
}

@article{musser1997introspective,
  title={Introspective sorting and selection algorithms},
  author={Musser, David R},
  journal={Software: Practice and Experience},
  volume={27},
  number={8},
  pages={983--993},
  year={1997},
  publisher={Wiley Online Library}
}

@article{rueckauer2016evaluation,
  title={Evaluation of event-based algorithms for optical flow with ground-truth from inertial measurement sensor},
  author={Rueckauer, Bodo and Delbruck, Tobi},
  journal={Frontiers in neuroscience},
  volume={10},
  pages={176},
  year={2016},
  publisher={Frontiers Media SA}
}
